Addressing interpersonal harm in online gaming communities: the opportunities and challenges for a restorative justice approach

Most social media platforms implement content moderation to address interpersonal harms such as harassment. Content moderation relies on offender-centered, punitive approaches, e.g., bans and content removal. We consider an alternative justice framework, restorative justice, which aids victims in healing, supports offenders in repairing the harm, and engages community members in addressing the harm collectively. To assess the utility of restorative justice in addressing online harm, we interviewed 23 users from Overwatch gaming communities, including moderators, victims, and offenders; such communities are particularly susceptible to harm, with nearly three quarters of all online game players suffering from some form of online abuse. We study how the communities currently handle harm cases through the lens of restorative justice and examine their attitudes toward implementing restorative justice processes. Our analysis reveals that cultural, technical, and resource-related obstacles hinder implementation of restorative justice within the existing punitive framework despite online community needs and existing structures to support it. We discuss how current content moderation systems can embed restorative justice goals and practices and overcome these challenges.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> comment.tex <==
%% comments
\definecolor{MyDarkBlue}{rgb}{0,0.1,1}
\definecolor{MyDarkGreen}{rgb}{0.02,0.6,0.02}
\definecolor{MyDarkRed}{rgb}{0.8,0.02,0.02}
\definecolor{MyDarkOrange}{rgb}{0.40,0.2,0.02}
\definecolor{MyPurple}{RGB}{111,0,255}
\definecolor{MyRed}{rgb}{1.0,0.0,0.0}
\definecolor{MyGold}{rgb}{0.75,0.6,0.12}
\definecolor{MyDarkgray}{rgb}{0.66, 0.66, 0.66}

\newcommand{\ns}[1]{\textcolor{MyRed}{[Niloufar: #1]}}
\newcommand{\sj}[1]{\textcolor{MyDarkBlue}{[Shagun: #1]}}
\newcommand{\sx}[1]{\textcolor{MyDarkGreen}{[Sijia: #1]}}


\newcommand{\ed}[1]{\textcolor{MyDarkBlue}{#1}}
\newenvironment{thisnote}{\par\color{MyDarkBlue}}{\par}




==> drafts/discussion_copy.tex <==
%this copy is newer

% \sx{hurt ppl hurt ppl - survey study}
% \sx{They were concerned with the restorative justice process because they were not sure whether the extra labor would make any changes.}

% \sx{problems in moderation model
% lack of accountability - favor offender
% does not address needs of support and healing and help offenders take accountability
% }

% \sx{cite institutionalized mediation in Slack; cite Discord moderator academy}
% \sx{Moderation is both top-down and bottom-up. - The Virtues of Moderation by James Grimmelmann }

\section{Discussion}


% We find both potentials and challenges for applying restorative justice values and practices in online communities. Some moderation practices have elements of restorative justice, and many moderators are strongly motivated to address the needs of the victims and the offenders to maintain a healthy community environment. Several victims and offenders are interested in participating in a restorative justice process. At the same time, many victims, offenders and moderators have concerns using the process in the harm cases they have experienced or addressed.

In this section, we first discuss how restorative justice principles may add to our understanding of the current practices of content moderation, which mainly have a punitive justice orientation. Next, we offer some possible ways for online communities to shift the current moderation practices to more restorative ones. Finally, we discuss the potential challenges in implementing restorative justice online and the resources needed to address them.



\subsection{The role of restorative justice in the moderation landscape}

Content moderation systems usually address online harm with a punitive approach. Yet, in our research, we found instances where this approach does not effectively meet the needs of victims or stop the perpetuation of harm from the offenders.
% Victims often do not engage with the decision-making process of moderation; thus they are deprived of agency to address harm and do not receive the support they need to heal. When the moderation system is centered on punishment, it is ineffectual in motivating changes to the offending behaviorsxi, and technical affordances allow offenders to easily sidestep punishments \cite{kou2021punishment}. In this punitive system, moderators and community members can also further perpetuate the harm by being unsupportive towards the victims and punitive towards the offenders.
Restorative justice provides a set of principles and practices that has the potential to address these issues by centering victims' needs for support and healing, and encouraging offenders to learn from their wrong-doing and take accountability. Through mediating conversations with victims and offenders, restorative justice facilitators support victims to share their feelings and receive support. It also provides offenders a chance to learn their wrong-doing through listening to the victims' narratives and encouraging them to change. Table \ref{table:2} compares the values and practices of the punitive content moderation approach in our sample with restorative justice. 


\begin{table*}
\setcounter{table}{1}
\centering
\begin{threeparttable}
\caption{
In this table, we compare restorative justice approach and the punitive content moderation approach in our sample.
}
 \label{tab:commands}
\begin{tabular}{p{5cm}|p{7cm}}
% \midrule
% \textbf{Addressing online harm} \\

\midrule
\textbf{Punitive content moderation approach} & \textbf{Restorative justice approach} \\
\midrule
Does not include victims in the process of addressing harm.	&
% Understand and validate victims' experiences, p
Provides victims with an opportunity to determine what they need from the offender and the community to address the harm (e.g., understand and communicate with offenders, an apology). 	\\ \hline
Regulates offenders through punishment and rule-centered explanations.	&	
Encourages offenders to realize the impact of their actions and take responsibility to repair the harm. \\ \hline
Does not include community members in the process of addressing harm. & Engages community members in supporting victims and offenders and heal collectively.
	\\ 
\midrule
 \end{tabular}
  \label{table:2}
  \end{threeparttable}
\end{table*}

We argue that whether to apply restorative justice in an online community is a value related question. While restorative justice and punitive justice processes have the shared goal of addressing harm and preventing the perpetuation of harm, they have different processes and orientations towards when justice is achieved. Content moderation---closer to a punitive justice approach---addresses harm through placing limits on the types of content that remain on the site and punishing offenders in proportion to their offense. Restorative justice, on the other hand, aims to assure that victims' needs are met, and offenders learn, repair harm, and stop offending in the future. Thus, the primary reason for applying restorative justice in moderation is not how it helps to achieve the current goals of effectively removing inappropriate content and punishing offenders, but how online communities may benefit from restorative justice values and goals. Recent research has argued that social media platforms have responsibility to achieve values instead of merely those that align with platforms' goals \cite{helberger2018governing}. In particular, some researchers have proposed values and goals that align with restorative justice, such as centering victims' needs in addressing harm \cite{schoenebeck2020drawing, blackwell2017classification}, democracy \cite{seering2020reconsidering}, and education \cite{myers2018censored}. Our research adds to this line of research and demonstrates how restorative justice may benefit online communities in addressing some severe forms of online harm such as harassment.

Restorative justice is a voluntary process and whether to apply restorative or punitive justice in a particular harm incidence is also related to the values of the key stakeholders involved. In our interviews victims, offenders, and moderators have different conceptualizations of justice. Seering et al. found that community moderators have diverse values in what moderation should achieve \cite{seering2020metaphors}. While some have a more punitive mindset and hope to be a ``governor,'' others align more with restorative justice values and hope to be ``facilitator,'' or ``gardener.'' Thus, it is important for online platforms to reflect on their values and goals and decide on what mechanisms (e.g. whether punitive or restorative justice) help realize those values. Additionally, Schoenebeck et al. found that people's preferences of punitive or restorative outcomes vary with their identity or social media behaviors \cite{schoenebeck2020drawing}. It is thus equally important to attend to victims' and offenders' preferences in individual harm cases. 

Next, we talk about ways to adapt the current moderation practices and implement restorative justice in moderation to address online harm.

\subsection{Applying Restorative Justice in Online Moderation}
We found that many moderators we interviewed hold differing elements of restorative justice values and practices. Some moderators hope to support victims and give offenders a second chance but do not have the proper tools or procedures for it. Some moderators have practices that embed elements of restorative justice such as talking with offenders and victims. Two of them (P7, P25) have tried out restorative justice in their own online communities. We propose that moderators can utilize their existing moderation practices that partially align with restorative justice as a first step towards approaches that are more restorative. We offer some potential directions below.


\subsubsection{Embed restorative justice language in moderation explanations}
Moderators can embed restorative justice language in explanations of moderation decisions. Prior work has shown that providing explanations for moderation decisions can reduce re-offense in the same community, but many moderated offenders also dismiss such explanations and continue re-offending \cite{jhaver2019survey, jhaver2019transp}. In our research, we find that explanations often focus on describing community guidelines or presenting community’s norms to the users, but do not 
encourage offenders to reflect on the impact of their actions. These explanation usually indicate the actual or potential punitive consequence, which may direct offenders' attention to the moderation system instead of their victims. We suggest a shift in language from a rule-based explanation to an explanation that highlights the possible impact offenders may cause for victims and supports the offender in taking accountability. Facilitator P5 provided an example of how she would communicate with the offenders if she were an online facilitator: \textit{``This post had this emotional impact [\ldots] this is how you've caused harm. This is the feedback from the community, and we want to work with you to create change.''}

Additionally, victims are often left out of the moderation process in the online communities we studied. However, some victims want to get information on the moderation process and result.  While prior research has talked about how moderation transparency prevents offenders from re-offending \cite{jhaver2019transp}, our work points to the importance of providing information for victims in the moderation process. Besides, victims have needs for support and healing. We suggest that a note of care may help victims feel heard and validated and help them recover. 

\subsubsection{Restorative justice conferences with victims or offenders}
% In our interviews, we found that some victims or offenders may not be available or willing to meet and have a conversation to address the harm. When a collective conference is not possible, it is possible to apply a \textit{partial restorative justice process} that are with offenders or victims alone \cite{kuo2010empirical, mccold2000toward}. 

Some Discord moderators already talk with victims and offenders before making moderation decisions, a practice redolent of restorative justice pre-conferencing. In offline pre-conferencing, facilitators ask a series of questions to help victims and offenders reflect on the harm, which provides opportunities for healing and learning to them. We believe that pre-conferencing provides opportunities to meet some needs participants identified in the interviews. For example, some offenders want to issue an apology to the victims; victims may not want to meet offenders but just let their feelings be known. 

In offline restorative justice, pre-conferencing is a preparation step for a potential victim-offender conference. Thus, if both victim and offender indicate willingness to meet with each other in the pre-conference, the moderators can organize a victim-offender conference, where victims and offenders share their perspectives and collectively decide how to address the harm. Moderators have the responsibility to maintain a safe space for sharing, for example, to halt the process when harm seems likely to happen, ensure a power balance between the victim and offender, and work with participants to establish agreements of behavior and values to adhere to throughout the process \cite{bolitho2017science}. In cases where restorative justice does not succeed, protection and preventing the continuation of harm might take a higher priority. Because facilitating those processes is difficult, we discuss the challenges and opportunities for moderators to facilitate in the following section.


A victim-support group is another form of restorative justice conferencing \cite{dignan2004understanding}. In our sample, many victims indicated a need for receiving emotional support. We propose that online communities can provide a space for victims to share the harm they experienced and receive support. Similar work has been seen in the online space. For example, Hollaback is a platform that allows victims of street harassment to empower each other through storytelling \cite{dimond2013hollaback}. Heartmob enables victims to describe their experiences of harm and solicit advice and emotional support from volunteer Heartmobers \cite{blackwell2017classification}. While those platforms are separate places from where harm happens, it is important to think about how online communities can support victims by motivating the community members to provide support.

% In our interviews, several victims and one offender showed willingness to use victim-offender conference to repair the harm.  As moderators we interviewed mentioned, confrontation may cause further harm to the victims. In offline restorative justice, facilitators follow a series of procedures to ensure the safety of victims (e.g., voluntary meeting, pause meeting when potential harm may happen) [cite]. 

We have so far illustrated why a restorative justice approach may provide advantages over the current punitive system. Yet, our intention is not to advocate for restorative justice as a wholesale replacement of the current moderation approach. Participating in restorative justice processes is voluntary. We propose that restorative justice goals and practices be embedded as part of overall governance structures in online spaces. For instance, restorative justice conferencing should only be used in select cases. A larger governance structure should take into account what to do if restorative justice processes fail. For instance, if it is determined at the pre-conference stage that a restorative justice approach cannot be applied, actions such as removing access by muting or banning might be used to prevent the continuation of harm. This is consistent with offline restorative justice practices, where the community or court clearly defines the types of cases that go through a restorative justice process and the action to take if a restorative justice process is not possible \cite{gavrielides2017restorative, van2016overview}.

\subsection{Challenges in Implementing Restorative Justice Online}
Applying restorative justice practices online is promising, but not straightforward. Though it has the potential to stop the perpetuation of harm and to improve community culture in the long run, there are structural, cultural, and resource-related obstacles to implementing a new approach within the existing punitive framework. Changing those conditions requires effort and resources from the platform, moderators, and community members. Here, we detail potential challenges of implementing restorative justice online and possible ways to address them. 

\subsubsection{Labor of restorative justice}
Shifting to a restorative justice process requires significant labor from online communities. The first source of labor comes from the training of facilitators. Unlike punitive justice, restorative justice is not currently a societal norm that people experience and learn on a daily basis. Aspiring facilitators need to receive additional training to learn restorative justice principles and practices to carry it out successfully and without causing more harm. Second, restorative justice conferences can be time intensive for all stakeholders involved. Before victims and offenders can meet, facilitators have to negotiate with each party in pre-conferences, sometimes with multiple rounds. The collective meeting involves a sequence of procedures, including sharing, negotiating and reaching consensus. Stakeholders, in particular facilitators, must expend emotional as well as physical labor. In offline practices, facilitators usually occupy a paid role in organizations \cite{gavrielides2017restorative}. The voluntary nature of moderation on social media sites like Discord means that facilitators may be asked to do extra unpaid work. This issue can be particularly salient when moderators already expend extensive physical and emotional labor with the ever expanding community scale \cite{roberts_behind_2019, dosono2019moderation, steiger2021psy}.

It is thus important for online communities to allocate resources to address the labor issues, which could come from both the top down and the bottom up. A top-down process requires resources from companies that host online communities. In the offline world, the successful implementation of a restorative justice mechanism usually requires institutional input \cite{gavrielides2017restorative, bazemore2001comparison}. The institution has the power to establish restorative justice as part of the official regulation process, provide resources to train and support the community members who want to become facilitators, and hire professional facilitators. Similarly, the companies that host online communities could provide those resources. There is some precedent for platforms making such investments---in recent years, social media companies such as Discord have hosted training for its community moderators \footnote{Discord Moderator Academy. https://discord.com/moderation}.
The bottom-up process engages users with preexisting knowledge about restorative justice to first try out the process and gradually expand the culture and practice. Offline restorative justice developed and evolved through local communities all around the world \cite{zehr2015little}. In our sample, two moderators have attempted or practiced online restorative justice within their own communities. They showed enthusiasm for expanding restorative justice practice in online gaming communities. We believe that input from companies and practitioners could collectively begin to address the labor problem. 

In addition, we see restorative justice as a re-allocation of labor instead of merely an addition of labor. Several moderators in our sample told us that they spend extensive amounts of time to make sure that the punishment they mete out is in proportion to the offense. Many of them also provide moderation explanations to offenders. Restorative justice, instead of requiring a new procedure, asks for a shift of purpose of those processes from determining offense to caring for victims and offenders.
In addition, if online restorative justice can stop the perpetuation of harm more frequently than punitive justice, it can reduce the need for moderation labor in the long term. While research has shown that offline restorative justice has successfully reduced re-offense rates \cite{latimer_effectiveness_2005, morris1993giving, daly_restorative_2002}, how restorative justice may work out in online communities and its effectiveness is an important area for future work.

\subsubsection{Offender accountability}
Another challenge may be in motivating offenders to take accountability for their wrong-doing. In our interviews, we found that with the technical affordances and moderation scope, offenders may easily avoid any consequences. The harm may happen in a place without moderation or clear rules of moderation (e.g., if harm occurs during a private chat in Discord, or happens across multiple platforms). Some participants also noted that it is easy to have multiple identities in Overwatch or Discord. Thus, when punishment is not effective, punitive justice may also lose its effectiveness.

Punishment is not the only form of holding offenders accountable. Restorative justice believes that people are not regulated only by punishment; they are also tied through relationships. Our interview data as well as restorative justice literature suggest the importance of community building---if offenders perceive themselves to be members of a shared community with victims, they will be more likely to take accountability to address harm \cite{pranis2015little, karp_restorative_2001}. It is equally important to have a shared list of community values and agreement on restorative justice processes to clearly define accountability. However, in our interviews, we find that there is a lack of sense of community. Offenders may not expect to meet victims again or hide behind multiple anonymous accounts. Moderators typically moderate a confined space of general chat, which can leave harm unaddressed in any places outside.

We argue that it is important to inquire into what accountability means to the community and how to hold people accountable in the current online moderation system. If offenders can simply avoid any consequences of conducting harm and do not feel a sense of belonging to the community where harm occurs, it would be challenging to engage them in any process---punitive or restorative---that holds them accountable. 

% In our interviews, moderators expressed concerns about whether the proposed new process would fail, for example, whether offenders would be disingenuous during the meeting or re-offend after the process. It is true that not all restorative justice sessions can achieve the desired outcomes. We now discuss some potential outcomes of a restorative justice process, potential failures in implementing it online, and ways to address these issues.

% Further, we argue that communities should be cautious about expecting or enforcing a positive outcome. Enforcing forgiveness from victims or expecting a change in offenders' behavior may undermine victims' needs and put them in a vulnerable place for forgiveness or induce a disingenuous response from the offenders \cite{bazemore2015restorative}. Online communities should allow for partial success or no success without enforcing the ideal outcome, especially at the early stage of implementation when there are insufficient resources or commitment. Instead, communities should maximize how victims, offenders and the entire community could benefit from the process.

\subsubsection{Emotion sharing and communication in restorative justice}
The limited modes of interaction and the issue of anonymity of online platforms may influence the effectiveness of restorative justice. Many online interactions are restricted to text or voice, which prohibits victims and offenders from sharing emotions, and may give rise to disingenuous participation. Emotional engagement by victims and offenders is essential for empathy and remorse \cite{strang2003repairing}. Face-to-face sharing enables victims and offenders to see each other's body language and facial expression. Besides, offline restorative justice has a series of physical structures and meeting procedures to elicit genuine, equal sharing. For example, participants sit in a circle; individuals who speak hold a talking stick; there are rituals at the beginning of the conference to build connections among participants and mark the circle as a unique space for change \cite{pranis2015little}. Those conditions for emotion sharing are hard to replicate in the online space. For example, if an offender messages an apology through text, it can be harder to discern a genuine apology from a disingenuous one. 

Disingenuous engagement is always possible, in particular in the online space when there are limited modes of interaction and a lack of accountability. Though disingenuity may exist, its cost can be high. The restorative justice process, especially the conference, should not be seen as an easier process for offenders to escape from punishment. Restorative justice requires time and effort to acknowledge one’s wrong doing and on actions to repair the harm, which is not a necessity in punitive justice \cite{zehr2015little}. Offenders may not see those actions to repair harm (e.g. community service) as an easier option compared to punitive processes \cite{wodahl2013offender}. Restorative justice gives people the benefit of the doubt. As practitioner Braithwaite noted, \textit{``Restorative justice is not about picking good apples for reconciliation and bad apples for deterrence; it is about treating everyone as a good apple as the preferred first approach''} \cite{braithwaite1999restorative}. Restorative justice is not about proving or testing the authenticity of offenders; it is about providing space and support for them to genuinely want to repair the harm. It could even be a space for identifying the disingenuity and work on them, which is a key step towards offenders' change and what victims may hope for.

The issue of computer-mediated communication and emotion-sharing has been long-discussed in HCI and CSCW literature. In recent years, increasingly more advanced technologies are being developed to facilitate civil engagement and communication in online systems. For example,
Kriplean et al. built a platform, ConsiderIt, to support reflective interpersonal deliberation \cite{kriplean2012}.
REASON (Rapid Evidence Aggregation Supporting Optimal Negotiation) is a Java applet developed to improve information pooling and arrive at consensus decision \cite{introne2008adaptive}. 
% Zhang et al. developed a Digital Jury to facilitate democratic moderation decision-making process [cite]. 
Many researchers have attempted to model human-like characteristics and emotional awareness in chatbots \cite{adikari2019cognitive,spring2019empathic}. In the context of restorative justice approach, Hughes has developed a tool, Keeper, for implementing online restorative justice circles \cite{hughes2020keeper}. Such existing systems can be leveraged to develop tools that facilitate emotion-sharing and communication in online restorative justice processes.
% \sx{Shagun, any other work you would suggest? There are so many works in CMC}
% \sx{to do: what are some works abt emotional sharing?}

\subsubsection{Expanding people’s notion and understanding of justice}
We believe that one crucial step toward successfully applying alternative justice frameworks (e.g. restorative justice) online is to expand people’s notion and understanding of justice. Before people can imagine and implement the alternative justice frameworks to address harm, they need to be aware of them. However, we found that although people have needs that the current system does not address, their options and mindset are often limited to what the current system can achieve through its punitive approach. As our research shows, many moderators and victims think that punishing offenders is the most or best they can do, and some offenders also expect to receive punishment. Some community members may further perpetuate the punishment paradigm. This mindset is not only a result of the gaming community’s culture; the punitive mindset is pervasive because of its widespread application throughout society, including in prisons, workplaces, and schools \cite{foucault_discipline_2012, king2009conservative}. 

While this research focused on the restorative justice approach, it is not the only alternative and has its limitations. Expanding people's notion and understanding of justice creates opportunities to utilize the strengths of different justice frameworks.  
% While this research focused on the restorative justice approach, we note that it is not the only justice model that can be used to address online harm. 
As some of our participants mentioned, many harms are rooted in structural issues such as sexism and racism. Effectively addressing such issues requires a deep, collective commitment to transforming the underlying conditions that enable harm to occur. Transformative justice \cite{daly2001transformative} and community accountability \cite{molyneux2012community} are some of the frameworks of justice that have been developed for this purpose. We believe that the work of transforming the underlying conditions that foster harm must simultaneously be done by everyone and in all communities for a sustained change to occur.

Expanding people’s notion and understanding of restorative justice can help avoid the mistrust and misuse of this approach. In our analysis, we found that participants' resistance to restorative justice can come from misunderstandings. Many participants we talked to are concerned about the labor of a victim-offender conference; while the concern is valid, communities can being by implementing partial processes that require less labor (e.g., changing language of moderation explanations). Some offenders in our interviews were reluctant to engage in restorative justice because they still expected to receive bans after the process, but restorative justice usually serves as an alternative to instead of an addition to punishment. We found that such concerns usually lead to quick rejections of the notion of online restorative justice. Helping people understand the diversity of restorative justice processes and how its aim is restoration instead of punishment may ease those doubts and open more opportunities for change. Besides, incomplete understanding of restorative justice may cause harm in its implementation. For example, enforcing ``successful outcomes'' may disempower victims and result in disingenuous responses from offenders. 
% Its core value is reparation of harm; 
Adapting restorative justice to online communities may require changes in format and procedure, but holding its values in mind may help avoid additional unintentional harm.

Finally, restorative justice has developed and evolved in practice \cite{zehr2015little, daly2001conferencing}, and it is important for people to experience it themselves in order to understand it, adapt it to their needs, and learn about its effectiveness. By experiencing it offline, several participants in our sample came to see it as a natural tool that can be adapted to online communities. In future work, we hope to pilot online restorative justice sessions and run survey studies to understand the types of harm that are more likely to benefit from restorative justice and the types of processes that would be useful. We would also like to provide more precise empirical guidelines about how restorative justice can be embedded in moderation systems. To manifest a future of restorative justice, \textit{``we will figure it out by working to get there''} \cite{kaba_2021}.

\subsection{Limitations and Future Work}
Our study has some methodological limitations. We used convenience and snowball sampling to recruit participants in one gaming community. As a result, our participants' experiences are not representative of all types of harm online. While Overwatch has a multinational and multicultural userbase, most of our participants are English-speakers from western cultures. In future work, we would like to conduct large-scale surveys to understand population-wide needs for a restorative justice process in addressing online harm.

In the study, we examined the possibility of restorative justice approaches in addressing harm in two ways. First, we analyzed the current moderation practice with restorative justice principles proposed by Zehr \cite{zehr2015little}. Second, we studied victims', offenders' and moderators' preferences for a victim-offender conference, one common restorative justice practice. There are diverse values and practices in restorative justice all over the world and they are evolving rapidly. We believe that future research can build on and expand restorative justice beyond the three principles and the victim-offender conference. In addition, while our research motivates a need for restorative justice, future research is needed to see how restorative justice can be integrated into an online community. In future work, we plan to collaborate with online communities to implement and test restorative justice practices.

\section{Conclusion} 
In this paper, we examined moderation practices in online gaming communities through the lens of restorative justice. We also studied the attitudes of different stakeholders towards implementing this framework in their communities. Our findings suggest that the values and practices of restorative justice has the potential to stop the cycle of harm and improve community culture in the long run. Much remains to be done for identifying the online spaces where this framework would be most beneficial and determining the best ways to implement it without face-to-face communication. We hope that this work serves as a useful guide for designers, volunteers, activists and other scholars to examine and implement restorative justice in online communities.

% When victims are not available, some offline conferences will invite surrogates (victims of similar types of harm) to join \cite{umbreit2007restorative}. We suggest that using surrogates in online restorative justice conferences is another possible way to improve offender awareness and reduce their recidivism. In our post-interview contacts with victims, several of them indicated a willingness to talk with offenders involved in other harm cases or send notes to share their feelings with the hope that it may change offending behavior.

% # how RJ
% ## how to implement
% Parital RJ

% RJ facilitator and moderator


% # challenges and preconditions
% accountability
% labor
% notion of justice


% Going into the moderation process/cycle of harm
% Offenders' tasks is to avoid punishment. Minimum cost -> punishment becomes a symbolic action
% Victims harm unaddressed. Next offender they meet is someone who avoided the last punishment
% Infuse more harm: punitive mind set to offenders

% ## Before applying RJ it's important to understand our values
% do we see addressing harm as part of the responsbility?

% ## One thing that is missing is accountability (for both punitive and restorative justice)
% Punishment is not the only accountability
% # moderation labor
% putting more resources in moderation
% stop re-offense, engaging other members in moderation

% ## The other thing is alternative ways to address harm
% Accountability 
% Cause of harm

% #there're things that punishment cannot achieve



% A lack of accountability favor offenders
% fact finding

% punishment does not work
% Problem of punishment
% Uncover what else can do

==> drafts/discussion_copy_2.tex <==
% from the intro of Race after Technology: "The dominant shift toward multiculturalism has been marked by a move away from one-size- fits-all mass marketing toward ethnically tailored niches that capitalize on calls for diversity."
% questions abt scale
%community has to be developed and fostered in intentional ways 
%define moderation sphere seems to be important
%ask julie: how does RJ deal with ingenuity?
% sense of community
%cite alex on scale thinking: technological solutions grounded in scale thinking are unlikely to be as liberatory or effective at deep, systemic change as their purveyors imagine.
%like mutual aid, RJ is anti-scale but it teaches people skills and give people tools to address their problems

%being a good facilitator requires lots of effort and training. I shouldn't down play it
%offenders seem reluctant to join. What should we do? We do we still think RJ is possible?

% should point out that there are many offline resources they can refer to

%need to be more conservative
% There are many elements of RJ in the current moderation process, it's just that the goals are different. Should utilize it in discussion


\sx{why RJ address those needs -> draw from paper}
\sx{relate to content moderation literature}
\sx{add in new citations in the recent two years}

\section{Discussion}
In this section, we first talk about how a restorative approach may help online communities address harm. Next, we offer some possible ways for online communities to shift the current moderation practices to more restorative ones. Finally, we then discuss the potential challenges in implementing restorative justice online and the resources needed to address them.

\sx{problems in moderation model
lack of accountability - favor offender
does not address needs of support and healing and help offenders take accountability
}
\sx{cite work on computer-supported communication and talk about how they have potentials to support the RJ process}
\subsection{Restorative justice complements punitive justice in addressing online harm}

The current moderation systems use punitive measures as the primary means to address online harm. Through a restorative justice lens, we found instances where the punitive approach doesn't effectively stop the perpetuation of harm. The victims do not receive the support and healing they deserve and it leaves them wounded. Sometimes, this sense of victimization may turn them into offenders who perpetuate the harm they once received. Although repeat offenders are banned from one community after a few rounds of graduated sanctions, they may re-offend with a new identity or in the next community they move to. 

% Moderators, as well as community members may further perpetuate the harm by being unsupportive to the victim or punitive to the offenders. 

Restorative justice provides an alternative and complementary way to stop the perpetuation of harm. We compared the values and practices of content moderation processes in our sample and restorative justice processes in Table \ref{table:2}. Through mediating conversations with victims and offenders, restorative justice facilitators support victims to address the harm and help offenders recognize the impact of their actions and take accountability. In our sample, several victims and offenders are interested in a restorative justice process. In addition, moderators have practices that embed elements of restorative justice such as talking with offenders and victims. 


\begin{table*}
\setcounter{table}{1}
\centering
\begin{threeparttable}
\caption{
In this table, we specify some of the ways that restorative justice facilitator's practice differ from a community moderator's practice.
}
 \label{tab:commands}
\begin{tabular}{p{6cm}|p{6cm}}
% \midrule
% \textbf{Addressing online harm} \\

\midrule
\textbf{Punitive justice} & \textbf{Restorative justice} \\
\midrule
Do not include victims in the process of addressing harm.	&
% Understand and validate victims' experiences, p
Provide victims with an opportunity to determine what they need from the offender and the community to address the harm (e.g., understand and communicate with offenders, an apology). 	\\ \hline
Regulate offenders through punishment and rule-centered explanations.	&	
%\sandy{I don't understand the following point....what does "meet offenders' needs for addressing harm" mean? Can you reword to clarify?}
% Understand and try to meet offenders’ needs for addressing harm (e.g., reparation of past harm or demonstrate change in front of the community).
Encourage offenders to realize the impact of their actions and take responsibility to repair the harm. \\ \hline
Address harm through making punitive moderation decisions. & Address harm through centering victims' needs for healing and offenders' need for learning.
	\\ 
\midrule
 \end{tabular}
  \label{table:2}
  \end{threeparttable}
\end{table*}

% have a shared goal of xxxx
% we do found that moderators and participants have different values of justice
% changing all people's notion of justice is out of scope for this paper

While restorative justice and punitive justice have the shared goal of stopping the perpetuation of harm and maintaining a healthy community environment, it is important to realize that the two justice frameworks have different understandings of when and how justice is done. Punitive justice address harm through punishing the offenders in proportion to the offense. On the other hand, restorative justice hopes that victims are healed, and offenders received learning and stop offending in the future. Thus, the primary reason for applying restorative justice in moderation is not how it helps to achieve the current goals of effectively removing content and punishing offenders, but how online communities may benefit from restorative justice values and goals. 

We believe that restorative justice or punitive justice are neither one-size-fit all approach. In our interviews, victims, offenders and moderators have different preferences for justice. Seering et al. showed how community moderators have diverse values in what moderation achieve [cite]. While some have a more punitive mindset and hope to be a "governor", some others align more with restorative justice values and hope to be "facilitator", "or gardener." Thus, it is important for online platforms to reflect on their values and goals in moderation and see whether punitive or restorative justice fits. Additionally, Schoenebeck et al. found that people's preferences of punitive or restorative outcomes vary with their identity or social media behaviors [cite]. It is thus equally important to attend to victims' and offenders' preferences in individual harm cases. 

Next, we talk about ways to implement restorative justice in moderation to address online harm.


% \sx{address how RJ reflect problems of current online communities more instead of directly advocating for RJ}

% It is also important to realize that restorative justice and punitive justice can achieve same outcomes in the process of pursuing justice. For example,  We showed how punitive justice failed to provide safety for victims in some cases when punishment loses its effectiveness. Restorative justice improve offenders' behaviors through building a sense of community and help them learn from their behavior. 

\subsection{Applying Restorative Justice in Online Moderation}
% \sx{acknowledge that left is punitive, right is restorative; and moderators may already have different notion of justice.}
For communities interested in restorative justice approach, we believe it is possible for moderators to align their values and practices with those of restorative justice facilitators. Online facilitators apply restorative justice principles in addressing online harm (Table \ref{table:2}). their actions and take accountability. 

% In addition, we believe that online facilitators should not make decisions for victims and offenders on how to address harm, in particular punitive moderation decisions. In our research, an offender tried to please moderator P7 during a restorative justice process, knowing that he can get unbanned with P7's moderation power. We believe focusing on needs to repair harm instead of punitive decisions can help offenders focus on addressing harm instead of potential punishment as well as provide victims more agency to meet their needs.

% We compared the values and practices of moderators in our sample and a proposed role of online facilitators in Table \ref{table:2}. 

Next, we outline some specific ways that online facilitators can implement restorative justice practices. We propose that online communities could begin with partial implementations and use existing moderation mechanisms as a gateway to practicing restorative justice. In addition, it is possible to hold victim-offender conference with willing victims and offenders.

% \begin{table*}
% \setcounter{table}{1}
% \centering
% \begin{threeparttable}
% \caption{
% We propose that moderators can shift from traditional, punitive moderation practices to restorative justice practices. In this table, we specify some of the ways that online restorative justice facilitator's role would differ from a community moderator's role.
% }
%  \label{tab:commands}
% \begin{tabular}{p{6cm}|p{6cm}}
% \midrule
% \textbf{Moderators} & \textbf{Online facilitators} \\
% \midrule
% Do not include victims in the process of addressing harm.	&
% % Understand and validate victims' experiences, p
% Provide victims with an opportunity to determine what they need from the offender and the community to address the harm (e.g., understand and communicate with offenders, an apology). 	\\ \hline
% Regulate offenders through punishment and rule-centered explanations.	&	
% %\sandy{I don't understand the following point....what does "meet offenders' needs for addressing harm" mean? Can you reword to clarify?}
% % Understand and try to meet offenders’ needs for addressing harm (e.g., reparation of past harm or demonstrate change in front of the community).
% Encourage offenders to realize the impact of their actions and take responsibility to repair the harm. 
% 	\\ \hline
% Make moderation decisions for victims and offenders.	&	Facilitate victims to reflect on and address their needs. Facilitate offenders to reflect on and take responsibilities to repair the harm.	\\
% \midrule
%  \end{tabular}
%   \label{table:2}
%   \end{threeparttable}
% \end{table*}

\subsubsection{Moderation explanation}
Online facilitators can embed restorative justice language in explanations of moderation decisions. Prior work has shown that providing explanations for moderation decisions can reduce re-offense in the same community, but many moderated offenders also dismiss such explanations and continue re-offending \cite{jhaver2019survey, jhaver2019transp}. In our research, we find that explanations often focus on explaining community guidelines present community’s norms to users, but do not educate offenders about the impact of their actions. We suggest a shift in language from a rule-based explanation to an explanation that highlights the possible impact offenders may cause for victims and supports the offender in taking accountability. Facilitator P5 provided an example of how she would communicate with the offenders if she were an online facilitator: \textit{``This post had this emotional impact [\ldots] this is how you've caused harm. This is the feedback from the community, and we want to work with you to create change.''}

% Additionally, though victims victims are left out of the moderation process in the online communities we studied. However, they have needs for support, healing, and information about the harm case they experienced. We suggest that a note of care from the moderators may help victims feel heard and validated and help them recover.

\subsubsection{Conferences with victims or offenders}
In our interviews, we found that some victims or offenders may not be available or willing to meet and have a conversation to address the harm. When a collective conference is not possible, it is possible to apply a \textit{partial restorative justice process} that are with offenders or victims alone \cite{kuo2010empirical, mccold2000toward}. 

Some discord moderators already talk with victims and offenders before making decisions. It is similar to pre-conference in restorative justice. In online pre-conference, facilitators ask a series of questions to help victims and offenders reflect on the harm, which provides healing or learning to them. We believe pre-conference provides opportunities to meet some needs participants identified in the interviews. For example, some offenders want to issue an apology to the victims; victims may not want to meet offenders but just let their feelings be known. In offline restorative justice, pre-conference is a preparation step of victim-offender conference. Thus, if both victim and offender indicate willingness to meet with each other in pre-conference, the online facilitator can organize a victim-offender conference. 
% It is worth mentioning that those conferences are not the end of restorative justice processes. The victim, community members as well as facilitators can provide support and acknowledgement when offenders carry out the action plans or changes that they have promised during the conference \cite{zehr2015little}.

% Pre-conference goes through a similar process as the following conference, where the victim or offender reflect on what has happened, how are people impacted and what is needed to repair the harm. The difference with conference is that either victims or offender in the harm is absent and the reaction from whom is hypothetical \cite{zehr2015little}.

Victim-support group is another form of restorative justice \cite{dignan2004understanding}. In our sample, many victims have the need for receiving emotional support. We propose that victims in different harm cases can join a conference to share the harm they experienced and support each other. Similar work has been seen in the online space. For example, Hollaback is a platform that allow victims of street harassment empower each other through storytelling\cite{dimond2013hollaback}. Heartmob allows victims to describe their experiences of harm and solicit advice and emotional support from volunteer Heartmobers \cite{blackwell2017classification}. While those platforms are separate places from where harm happens, it is important to think about how online communities can support their own victims by motivating the community members to provide support.

% In our interviews, several victims and one offender showed willingness to use victim-offender conference to repair the harm.  As moderators we interviewed mentioned, confrontation may cause further harm to the victims. In offline restorative justice, facilitators follow a series of procedures to ensure the safety of victims (e.g., voluntary meeting, pause meeting when potential harm may happen) [cite]. 

Restorative justice is not meant to replace the current governance process but is rather embedded as a part of the overall moderation process to handle selected cases. When the process cannot work out, punitive processes such as muting or banning are still available as backup options to stop the continuation of harm. This is consistent with offline restorative justice practices, where the community or court clearly defines the types of cases that go through a restorative justice process and the action to take if a restorative justice process is not possible \cite{gavrielides2017restorative, van2016overview}.


\sx{here: add more CSCW and CHI literature}

\subsection{Challenges in Implementing Restorative Justice Online}
Applying restorative justice practices online is promising, but not straightforward. Though we believe it has the potential to stop the perpetuation of harm and improve community culture in the long run, there are structural, cultural, and resource-related obstacles to implementing a new framework within the existing punitive framework. Changing those conditions may require effort and resources from the platform, moderators, and community members. Here, we detail potential challenges of implementing restorative justice online and possible ways to address those issues. 

\subsubsection{Labor of restorative justice}
\sx{cite content moderation literature on moderation labor, emotional labor}
Shifting to a restorative justice process requires significant labor from online communities. The first source of labor comes from the training of facilitators. Unlike punitive justice, restorative justice is not currently a societal norm that people experience and learn on a daily basis. Aspiring facilitators need to receive additional training to learn restorative justice principles and practices to carry it out successfully and without causing more harm. Second, restorative justice conferences can be time intensive for all stakeholders involved. Before victims and offenders can meet, facilitators have to negotiate with each party in pre-conferences, sometimes with multiple rounds. The collective meeting involves a sequence of procedures, including sharing, negotiating and reaching consensus. Stakeholders, in particular facilitators, must expend emotional as well as physical labor. In offline practices, facilitators are usually a paid role in organizations \cite{gavrielides2017restorative}. The voluntary nature of moderation on social media sites like Discord means that facilitators may be asked to do extra unpaid work. This issue is particular salient when moderators already pay extensive physical and emotional labor with the ever expanding community scale \cite{roberts_behind_2019, dosono2019moderation, wohn2019volunteer}.

\sx{joseph's work}
It is thus important for online communities to allocate resources to address the labor issues, which could come from both the top down and the bottom up. A top-down process requires resources from companies that host online communities. 
% In the offline world, the successful implementation of a restorative justice mechanism usually requires institutional input \cite{gavrielides2017restorative, bazemore2001comparison}. 
% The institution has the power to establish restorative justice as part of the official regulation process, provide resources to train and support the community members who want to become facilitators, and hire professional facilitators to do their jobs. Similarly, the companies that host online communities could provide those resources. 
The bottom-up process engages users with preexisting knowledge about restorative justice to first try out the process and gradually expand the culture and practice. In our sample, two moderators have attempted or practiced restorative justice within their own communities. They showed enthusiasm for expanding restorative justice practice in online gaming communities. We believe that input from  companies and practitioners could collectively begin to address the labor problem. 
%\sandy{Re preceding, wouldn't you have to make a business case for companies to make this investment? What are the companies' returns?}

\sx{modify the paragraph}
In addition, we see restorative justice as a re-allocation of labor instead of merely an addition to labor. Several moderators in our sample told us that they spend extensive amount of time to make sure that the punishment is in proportion to the offense. However, the process has similar elements to restorative justice (e.g. talking with victims and offenders, review offenders' activity history). Thus, we believe restorative justice reallocate the labor from determining offense to caring for victims and offenders. In addition, if online restorative justice can stop the perpetuation of harm more efficiently than punitive justice, it can reduce moderation labor though prevention of harm. How restorative justice may work out in online communities is important future work.

% In addition, our research shows that in a toxic community environment, it is not enough to address individual harm cases since new offenders will always come. Restorative justice has the potential to improve community environment and reduce offensive cases in the long run.

% We also believe that implementing restorative justice has the potential to reduce re-offenses and stop the perpetuation of harm, thereby reducing some labor needed for moderation in the long run. 
% Many proposed online restorative justice processes borrow elements from existing moderation practices (e.g. talking with victims and offenders, provide moderation explanations) and re-appropriate them with restorative justice values. 

% restorative justice may reduce some moderation labor required in the long term. First, restorative justice may seem to be a lot of work when people are not familiar with it. After making an effort to establish regular restorative justice practices with offline communities, members develop familiarity and acceptance with the conference process, which reduce the additional effort for learning how restorative justice works when using it \cite{karp_restorative_2001, bazemore1999restorative}. Second,  Third, 

%\sandy{Re previous argument, aren't moderators unpaid?  What's the net effect to companies, therefore, of having fewer of them?}

%\sx{facilitators will check whether offenders are genuine during the pre-conferencing}
\subsubsection{Technical affordances of online communities and platforms}
% In our interviews, moderators expressed concerns about whether the proposed new process would fail, for example, whether offenders would be disingenuous during the meeting or re-offend after the process. It is true that not all restorative justice sessions can achieve the desired outcomes. We now discuss some potential outcomes of a restorative justice process, potential failures in implementing it online, and ways to address these issues.
%addressing victims needs are also important so sometimes RJ uses partially admitted offenders!

% Before asking whether and how restorative justice could fail, we should define its criteria for success. Restorative justice has more expansive and diverse goals compared to those of traditional content moderation, which is usually to maintain the health of content. 

% Research shows that restorative justice performs better at reducing re-offense rates and increasing victim satisfaction and participants' perception of procedural justice \cite{latimer_effectiveness_2005, morris1993giving, daly_restorative_2002}.

The limited modes of interaction and the issue of anonymity of online platforms may influence the effectiveness of restorative justice. Many online interactions are restricted to text or voice, which prohibits victims and offenders from sharing emotions, and may give rise to disingenuous participation. Emotional engagement by victims and offenders is essential for empathy and remorse \cite{strang2003repairing}. Face-to-face sharing enables victims and offenders to see each other's body language and facial expression. Besides, offline restorative justice has a series of physical structures and meeting procedures to elicit genuine, equal sharing. For example, participants sit in a circle; individuals who speak hold a talking stick; there are rituals at the beginning of the conference to build connections among participants and mark the circle as a unique space for change \cite{pranis2015little}. Those conditions for emotion sharing are hard to replicate in the online space. For example, if an offender messages an apology through text, it can be harder to discern a genuine apology from a disingenuous one compared to offline scenarios. Further research can investigate how to implement digital analogues of such rituals and create a safe and helpful space for online sharing \cite{hughes2020keeper}.
Importantly, offline restorative justice can still be implemented for addressing cases of online harm when the stakeholders involved are physically co-located. 

\subsubsection{offender accountability}
Another challenge may be in motivating offenders to take accountability for their wrong-doing. In our interviews, we found that with the technical affordances and moderation scope, offenders may easily get away with any consequences of conducting harm. The harm may happen in a place without moderation or clear rules of moderation (e.g., if harm occurs during a private chat in Discord, or happen across multiple platforms). Some participants also noted that it is easy to have multiple identities in Overwatch or Discord. If offenders can simply avoid any consequences in conducting harm, it can be challenging for them to engage in any processes to take accountability --- no matter punitive or restorative. While punitive justice tries to use moderation to hold offenders accountable, restorative justice believes that people are not regulated only by rules: they are also tied through relationships. Our interview data as well as restorative justice literature suggest the importance of community building: if offenders perceive themselves to be members of a shared community with victims, they would be more likely to address the harm successfully \cite{pranis2015little, karp_restorative_2001}. It is equally important to have a shared list of community values and agreement on restorative justice processes to clearly define accountability in restorative justice processes. 
% In cases where restorative justice does not succeed, protection and preventing the continuation of harm might take a higher priority.


% We argue that it is important to inquire into what accountability means in the current online moderation system: 

% Disingenuous engagement is always possible, in particular in the online space when there are limited modes of interaction and a lack of accountability. However, the restorative justice process, especially the conference, should not be seen as an easier process for offenders to escape from punishment. Restorative justice requires time and effort to acknowledge one’s wrong doing and on actions to repair the harm, which is not a necessity in punitive justice \cite{zehr2015little}. Offenders may not see those actions to repair harm (e.g. community service) as an easier option compared to punitive processes \cite{wodahl2013offender}. Disingenuity may exist, but its cost can be high. Restorative justice gives people the benefit of the doubt. As practitioner Braithwaite noted, \textit{``Restorative justice is not about picking good apples for reconciliation and bad apples for deterrence; it is about treating everyone as a good apple as the preferred first approach''} \cite{braithwaite1999restorative}. Restorative justice is not about proving or testing the authenticity of offenders; it's about providing space and support for them to genuinely want to repair the harm. It could even be a space for identifying the disingenuity and work on them, which is a key step towards offenders' change and what victims may hope for.

% Further, we argue that communities should be cautious about expecting or enforcing a positive outcome. Enforcing forgiveness from victims or expecting a change in offenders' behavior may undermine victims' needs and put them in a vulnerable place for forgiveness or induce a disingenuous response from the offenders \cite{bazemore2015restorative}. Online communities should allow for partial success or no success without enforcing the ideal outcome, especially at the early stage of implementation when there are insufficient resources or commitment. Instead, communities should maximize how victims, offenders and the entire community could benefit from the process.

% [did not address what if they re-offense after RJ]

\subsubsection{Expanding people’s notion and understanding of justice}
\sx{mention how community members perpetuate harm}
We believe that one crucial step toward successfully applying alternative justice frameworks (e.g. restorative justice) online is to expand people’s notion and understanding of justice. Before people can imagine and implement the alternative justice frameworks to addressing harm, they need to be aware of them. However, we found that although people have needs that the current system does not address, their options and mindset are often limited to what the current system can achieve through its punitive approach. As our research shows, many moderators and victims think that punishing offenders is the most or best they can do, and some offenders also expect to receive punishment. Some community members may further perpetuate the punishment paradigm. This mindset is not only a result of the gaming community’s culture; the punitive mindset is pervasive because of its widespread application throughout society, including in prisons, workplaces, and schools \cite{foucault_discipline_2012, king2009conservative}. 

While this research focused on the restorative justice approach, it is not the only alternative and has its limitations. Expanding people's notion and understanding of justice creates opportunities to utilize the strengths of different justice frameworks.  
% While this research focused on the restorative justice approach, we note that it is not the only justice model that can be used to address online harm. 
As some of our participants mentioned, many harms are rooted in structural issues such as sexism and racism. Effectively addressing such issues requires a deep, collective commitment to transforming the underlying conditions that enable harm to happen. Transformative justice \cite{daly2001transformative} and community accountability \cite{molyneux2012community} are some of the frameworks of justice that have been developed for this purpose. We believe that the work of transforming the underlying conditions of harm must simultaneously be done by everyone and in all communities for sustained change to occur.

Expanding people’s notion and understanding of restorative justice can help avoid the mistrust and misuse of it. In our analysis, we found that participants' resistance to restorative justice can come from misunderstandings. Many participants we talked to are concerned about the labor for a victim-offender conference; while the concern is valid, communities can implement partial processes that require less labor (e.g., changing language of moderation explanations). Some offenders in our interviews were reluctant to engage in restorative justice because they still expected to receive bans after the process, but restorative justice usually serves as an alternative instead of an addition to punishment. In our research, those concerns usually result in quick rejections of the notion of online restorative justice. Helping people understand the diversity of restorative justice processes and how its aim is in restoration instead of punishment may ease those doubts and open more opportunities for change. Besides, incomplete understanding of restorative justice may cause harm in implementation. For example, enforcing ``successful outcomes'' may disempower victims and result in disingenuous responses from offenders. Its core value is reparation of harm; adapting restorative justice to online communities may require changes in format and procedure, but holding its values in mind may help avoid additional unintentional harm.

Finally, restorative justice has developed and evolved in practice \cite{zehr2015little, daly2001conferencing}, and it is important for people to experience it themselves in order to understand it, adapt it to their needs, and learn about its effectiveness. By experiencing it offline, several participants in our sample came to see it as a natural tool that can be adapted to online communities. In future work, we hope to pilot online restorative justice sessions and run survey studies to understand the types of harm that are more likely to benefit from restorative justice. We would also like to provide more precise empirical guidelines about how restorative justice can be embedded in the moderation systems. To depict a future of restorative justice, \textit{``we will figure it out by working to get there''} \cite{kaba_2021}.


% It has been implemented in many offline settings and offered as an alternative to punitive justice \cite{van2016overview,wood2016four}. 

\section{Conclusion} 
In this paper, we examined moderation practices in online gaming communities through the lens of restorative justice. We also studied the attitudes of different stakeholders towards iimplementing this framework in their communities. Our findings suggest that the values and practices of restorative justice has the potential to stop the cycle of harm and improve community culture in the long run. Much remains to be done for identifying the online spaces where this framework would be most beneficial and determining the best ways to implement it without face-to-face communication. We hope that this work serves as a starting point for designers, volunteers, activists and other scholars to examine and implement restorative justice in online communities.

% When victims are not available, some offline conferences will invite surrogates (victims of similar types of harm) to join \cite{umbreit2007restorative}. We suggest that using surrogates in online restorative justice conferences is another possible way to improve offender awareness and reduce their recidivism. In our post-interview contacts with victims, several of them indicated a willingness to talk with offenders involved in other harm cases or send notes to share their feelings with the hope that it may change offending behavior.

=======================================================

% # how RJ
% ## how to implement
% Parital RJ

% RJ facilitator and moderator


% # challenges and preconditions
% accountability
% labor
% notion of justice


% Going into the moderation process/cycle of harm
% Offenders' tasks is to avoid punishment. Minimum cost -> punishment becomes a symbolic action
% Victims harm unaddressed. Next offender they meet is someone who avoided the last punishment
% Infuse more harm: punitive mind set to offenders

% ## Before applying RJ it's important to understand our values
% do we see addressing harm as part of the responsbility?

% ## One thing that is missing is accountability (for both punitive and restorative justice)
% Punishment is not the only accountability
% # moderation labor
% putting more resources in moderation
% stop re-offense, engaging other members in moderation

% ## The other thing is alternative ways to address harm
% Accountability 
% Cause of harm

% #there're things that punishment cannot achieve



% A lack of accountability favor offenders
% fact finding

% punishment does not work
% Problem of punishment
% Uncover what else can do

==> drafts/draft.tex <==
% \sx{it's hard to find offenders}
% \sx{potential offenders}
% In our sample, we recruited offenders \ns{should we call them offenders? maybe potential offenders?} among people that have been banned or punished in other ways in Discord and Overwatch. When asked about their preference for a restorative justice process, some offenders showed willingness to join because they believed that they have received unfair moderation decision and wanted a chance to voice themselves. Among them, some think that they have also caused harm in the process \ns{what process} and are willing to take partial accountability. Several offenders are not willing to join the meeting because \ns{probably expain why} [fill later].

% Some offenders are willing to join the meeting when they think they are the victims of harm {mention moderators}. In offline restorative justice conference, offenders should agree that they have caused some levels of harm to the victims and show willingness to repair the harm \ns{they don't necessarily need to completely agree, that's why there's a whole process and pre-conferencing, for the offender to understand the impact of their actions is part of the process}[cite]. 
% {mine is not technically preconferencing}


% {divide the paragraphs through deeper findings}

% Though some offenders agreed to take partial accountability, they think the other side has also caused harm. They are motivated to meet with the victims because they want to use the meeting to justify themselves and punish the other side who was involved in the harm case.  Alpha was once banned in Overwatch for flaming\ns{what's flaming} other people. However, he thinks the other side initiated the fight and he defended himself for a justified reason. Alpha wanted to use the meeting as a chance to challenge the other side who caused his ban: ``So why is it I'm being reported and banned after saying one thing but yet you're not getting any punishments?'' Alpha believed that the one who caused him fight should be banned as well \ns{I don't understand this example, what's the higher level point you're trying to make here?}. 

% Some offenders are willing to take accountability to repair the harm when the harm is impulsive \ns{what's an impulsive harm? what's the alternative?} and they want to maintain a long term relationship with the victims. Will attacked Juba in the general chat. He admitted that he was emotional at that moment: ``I'm quite a stubborn person, as I said, and I was in the head space, I wanted to get the last word in, basically.'' He wished to repair their relationships: ``I would literally just settle for being civil with one another...And we don't have to be close friends at all. But as long as I know that if we're in the same voice chat or text chat together there's not going to be any animosity.'' \sx{is the case below good or bad?} In another case \ns{what's the purpose of another case? what points does it demonstrate?}, Fogi successfully organized a restorative justice conference with two of her gamer friends. The two gamers attacked each other under alternative accounts in an Overwatch game but found out they were friends afterwards. According to Fogi, both of them were hurt: ``They got really hurt about it and they kind of were really at feud with each other.'' They showed willingness to join the restorative justice meeting and was able to resolve the issue. In the meeting, both of them agreed that they wouldn't attack each other if they knew they were friends, and apologized to each other. \ns{this reads like a lot of back and forth between people I don't know and I'm not sure why I'm reading it}
% \sx{I've presented a strong casual relationship in this paragraph and with somewhat indirect examples, not sure if it's valid or not}

% In our sample, several participants believed they were banned because the moderators has abused their power when they disagreed with them. For example, Nyhq thought the moderator treated the community members unfairly: ``He would single out other people who were weak-minded. Especially females unfortunately...and threaten them with kicking them, banning them etc., if he didn't get his way.'' Nyhq approached the moderator with other members who saw the same issue, but the moderator banned all of them out of the community. Will and Sykelone were moderators themselves but were banned by moderators of higher status when they disagreed with the way they managed the community. All participants who fall under this category didn't think they have caused harm to others. Since they were either friend with the moderators who banned them or other members in the community, they were hurt by the bans. Nyhq described his feelings: ``One minute you think of these people as your friends, and the next .... for it to just go away, it was almost soul shattering...I was deeply hurt.'' He believed there is a lack of accountability when moderators have harmed others: ``[When] the higher members of staff were involved, nothing could be done.'' Similar to the victims we described in [the last section], they have a need to share their feelings with the mods and understand the motives for their action. They also hope the moderators do not abuse their power in the future.
% \sx{several of those moderators who caused harm were actually admins. Do we want to explain the difference between mods and admins?}
% \ns{I was confused about why we're getting into so much detail about moderators all of a sudden}

% Some offenders are not comfortable with the idea of a meeting or do not think the meeting can lead to a desired outcome. They think the punishment they received were justified and would rather receive punishment than attending the restorative justice meeting. In case X, Azure was banned for attacking Fogi and also the Fogi's reveal also caused his damage in reputation. Reflecting back, he didn't think he would want to attend the restorative justice conference at that time: ``That sounds boring. That sounds like, `I don't want to do this. I'm not going to go in with an open mind so nothing will get done anyways.''' Azure reflected, ``Would an immature 16 year old teenager who's rebellious against his mom, he doesn't want to do the freaking dishes, do you think he'll want to sit in a call or a meeting with the person that he just harassed for the last 20 minutes and figure it out? ’’ Mail was banned for flaming others in a game. He believed that he would be punished anyways: ``If you know for a fact you're in the wrong, then there's no point in even talking, because you're going to get banned anyway.'' 




% \subsubsection{The community culture feeds into harm} \ns{in other words, the community isn't going to hold anyone accountable if the community is racist/sexist, etc.}



%Punishment is also a norm when people come across problems (notion of justice)
%Azure reflected on why he used to attack the victims: ``it's just because [the victim] is in our game and we're losing, so we're going to find something to blame it on, and since we're bullies, we're going to extend it beyond just the game…We're going to make sure that you feel like shit at the end of the game.’’

%The moderation and the community both use punishment as the main methods to address offenses. [expand or leave for Discussion?]





%\subsubsection{what is a community for moderators, victims and offenders}


%In one community we researched, the moderators have a different sense of community. The community help people create and organize regular teams to play in Overwatch. If there is any harm happens, the team can refer to the community lead to help solving the problem. According to Awanei, xxxxx.


%I think it was about a year ago. And what would happen was there would be problems in the community, but we wouldn't know about it. We do a pretty good job of skimming all the channels and reading up on everything to make sure everything's going well. But there was some stuff that would happen, invoice chats that we in, and people would start causing problems with each other. We wouldn't know about it and it would cause people to leave the community. 
%A really active member who'd been here for a while would just leave. And we were like, "Oh, why did you go?" And they were like, "Well, there was this thing, but I didn't want to make a problem about it or whatever, so I just left." And we're like, "Well, that's an easy fix if you tell us, but we can't do it unless you tell us." It happened two or three times and we said, "Okay, you guys are really concerned about your name's being attached to your complaint. We'll set this role up specifically for you guys to be able to bring your concerns too."

%we've also had people come ask us to ban somebody, where it's like, "Do you just want the ban because you don't like them? Whereas you can just go and block them and never have to speak to them again and they can't get ahold of you." (interview data and analysis\interview 14 Awanei: 288 - 288)


%also cite Bivi and Arca, they don't come across harm with friends
%It is possible that I could avoid harassment by just playing with my friends and not having random people on the team, but I think the main problem is that the teams are of six people and it's hard to get six people on playing the same game at the same time, because a lot of my friends are on different schedules, on different parts of the US. And I like to play more. I like to play a lot more than just when six people are available to play. So that's the only reason. (interview data and analysis\interview 11 Arca: 429 - 429)



%to discuss
%In Discord, moderators have the power to decide what happens to offenders. Several participants believe that they were wrongfully banned when the offenders are the moderators.\\

% \fbox{%
%     \parbox{\textwidth}{%
    
%     \textbf{Case 2} \\
%     Nyhq was once a member in a Discord community. He believed the admin has been abusive to certain members: “the admin would single out people and threaten them with kicking them, banning them etc., if he didn't get his way. People were friend with each other already so being kicked out of the group meant a great deal.”

%     Nyhq and his friends who were aware of the problem tried to negotiate with the admin, but Nyhq thought the admin saw it as a threat. The admin ceased all contact with them and banned them from all of the communities.

%     }%
% }\\

% Discord Moderator Louise described their principles: ``In general, the first defense for most things is a warning or mute…[if] they have been warned or muted before, that we'll start looking at temporary bans or permanent bans.''







% Though the harm emotionally impacts victims, offenders do not reflect on the harm they cause and feel the emotional impact \ns{there needs to be a sentence or two before this that explains why this is important. e.g. for the offender to hold themselves accountable and seek to make changes they need to understand the effects of the harm they caused (cite RJ)}. Azure used to harm others but has changed afterwards. He reflected, ``[The victims’] day is legitimately ruined because of what [offenders] said, but these people aren't going to think about what they said twice…They're not going to reflect because it doesn't affect them.’’




% ============= % ============= % ============= % ============= % ============= % =============
% \subsubsection{offenders do not have a chance to learn the impact of their actions and repair their wrong-doing}
% Restorative justice asks offenders to take accountability by listening to victims share their story, understanding the impact of harm, and changing behavior afterwards. Offenders sometimes repair harm by contributing to the community (e.g.doing community service) [cite]. If victims and offenders reach consensus on what is needed to repair the harm, the offenders receive no punishment or reduced punishment [cite]. We find that in both Overwatch and Discord, punishment is the major means to hold offenders accountable. As discussed in the previous section, punitive models are often insufficient to satisfy victims of online harm. At the same time, punishment does not effectively help offender change their behavior and prevent re-offending. Even in cases where offenders are forced to change their behavior, or prohibit from participating, they do not get a chance to understand their wrong-doing. 


% ============= % ============= % ============= % ============= % ============= % =============


% \fbox{%
%     \parbox{\textwidth}{%
    
%     \textbf{Case 2} \\
%     Azure and his friend were playing with a female player on their alternative Overwatch accounts that were not linked to their identity. He and his friend started to attack the girl after they lost the first round. Fogi, the girl played with Azure, decided to record the video and posted it on Twitter after the attack continued for a while: ``I knew that it was something that a lot of women and a lot of people deal with daily almost within the community. I wanted to be able to show just how bad it can be.'' Though Azure and his friend were using their alternative account to play, someone recognized their voice and revealed their main account. Their main account was temporarily banned as a consequence.

%     However, for Azure, the account banning was not the most severe punishment --- it was the following harassment and his ruin of reputation after the reveal. He reflected, ``I would get random messages throughout the day saying, `You should kill yourself,’ and death threats like, `I'm going to come. I will.’ He left his old online identity completely: ``I deleted my Twitter, deleted Instagram, deleted Discord, changed all my Overwatch account names.' Azure later apologized to Fogi and changed his behavior afterwards. However, as a 17-year-old, the incident permanently changed his career path: ``To be honest I think that was the main reason I didn't try to pursue to go pro in Overwatch harder...because of the reputation damage, and because of how much I had to do to get back on the reputation...I had to basically restart.''

%     Azure has changed his behavior afterward. While he was banned from the game and condemned by many gamers, Azure’s learning come from his friend. One of Azure’s friends reached out to him: ``he was like, `Dude this is going to sound harsh but you're going to need to hear it…The reason why you don't feel empathy for these people is because you don't interact (with people offline).'' At that time, Azure used to play video games all day after school. Azure took the advice: ``After school you gradually start to break out of your shell a little bit...Going outside, talking to real people and interacting with them face to face so you can see their emotion and how they react.'' As time went on, he started to feel the impact he created on others:  ``Now…I can imagine them sitting at their computer and just like crying, because they're sad about what I said, and that's why I don't say these things.''

%     }%
% }\\


% We find that the restorative justice approach and the current moderation system treat offenders differently. Restorative justice encourages offenders to change their behavior by helping them learn the impact of their actions \cite{zehr_little_2015}. In the victim-offender conference, the offenders hear the victims share their feelings; the facilitator also tries to convey the victims' side of the story to offenders \cite{johnstone_handbook_2013}. Restorative justice posits that such learning is essential to help offenders reflect on what triggers them to cause harm and prevent their future offenses. On the other hand, the current moderation system seeks to change offenders' behavior through punishment. 
% This system is characterized by graduated sanctions where offenders first receive lenient punishment (e.g., warning, muting, temporary ban), often without any explanations for such sanctions, before they are permanent banned from the community. Our participants noted that the punishments and explanations that characterize the current moderation system are centered around platform/community guidelines or rules.
% Though this approach can limit or even stop wrongful acts, it precludes many offenders from learning how their actions impact others or reflecting on why they caused harm. Further, it directs offenders' attention to the punishment and the moderation system instead of the victims and the consequences of their actions.

% According to Bivi, the bystanders also fuel into harm. 

% And the harm can expands to indirect victims. [Add: Azure shared the video in his Discord friend group so Arca saw it.] Arca reflected on her feelings after seeing the video of Azure attacking Fogi: “I was furious. I was so angry that he had done something like that.” Bivi described how she was affected by the video: “I was sickened by the things that he said to this girl...for me it reminded me of all the reasons I am afraid to speak in game. ”


% Victim Bivi talked about how the bans could not ease her feelings:  \textit{``I wish that (banning them) made me feel more comfortable but in this community, one account gets banned and they just buy a new one and don’t change.''} Several participants who have been banned confirmed the thoughts. Azure reflected, ``In actuality, when I got banned I'm going to say, `I don't give a fuck, I'm just going to log into my second account.''' 

% In Discord, offenders can also easily make a new account. However, while there are no mechanism for the moderation system in Overwatch to detect alternative account, moderators in Discord can recognize alternative account if they are familiar with the user. Moderator Paddington described how she identifies alternative accounts: ``People may recognize the voice, people may recognize their Overwatch user name, or it may be a known Overwatch account of theirs affiliated with that.''
% %The punishment turns the game between moderators and offenders, while the purpose of both sides becomes justifying their standpoint.

% In some communities, the offenders are hostile to the moderators. As moderator Sykelone reflected,``[As a moderator], you've got to be careful with where you step because seeing one wrong thing can just lead a witch hunt after you. (Sykelone)'' Victims are left out of the process, and the 

% We find that many offenders (P17, P19, P20, P21, P22,) are aware that they have caused some level of harm to others, but they acknowledge the impact of their action differently. Some participants regretted causing harm to others. For example, P22 regretted attacking a user in a Discord channel publicly and admitted that sometimes he failed to control his emotions: \textit{``I have an extremely competitive and stubborn personality so when something doesn’t exactly go to plan, it can be difficult for myself to accept and get over.''} On the other hand, several offenders believed that they defended themselves for a justified reason because others behaved improperly or have hurt their interest in the first place (e.g. when their teammate in Overwatch didn't play the game well or they witnessed a gamer bullying their friend). P19 talked about how he defended himself by intentionally hurting others' feelings: \textit{``Every single time I speak, I will make sure they feel small, helpless, defenseless, and worth nothing.''} 

% \sx{Two participants in our sample believe they were wrongfully banned because the moderators abused their power. Mention or not?}

% Offenders are often unwilling to repair the harm in offline restorative justice practices too. In such cases, alternatives measures are sought; victim-offender conferences only occur when both sides are willing to meet each other and address harm \cite{zehr_little_2015}. To understand the preferences of victims and offenders, the facilitator meets with each party in a preconference \cite{johnstone_handbook_2013} and determine if they are willing to meet and address the harm collectively. In cases where only victims are available, there can be other formats of meeting. For example, there can be meeting with surrogates (offenders from other cases), meetings where victims share their experiences with the community, or meetings where victims of different harm cases come together and share their experiences \cite{morris_restorative_2001}.

% =================


% how to use principles

% scale labor it requires time




% cycle of harm takes a lot of time
% enforcing the rules take a lot of time (Shagun, Joseph's paper)
% how do you enforce rules? Do you enforce rules by punishing people? Or restorative justice?
% It's about where we put our resources
% It's an open question whether we will spend more labor in the long term



% Does the current research address community culture and re-offense?

% restorative justice can stop reoffense
% restorative justice's labor?

% Don't start with implementing
% Can we argue that the community now can start to implement restorative justice?



% open up the alternatives
% talk about how it was implemented in offline

% not ready to implement yet

% most direct potential 

% calling for activists to make changes
% starting from communites that are more receptive to those ideas

% young people may benefit








% There are existing preconditions for victim-offender conference. The 
% current literature: how many are about addressing reoffenses?



% [restorative justice is a possible way to address the issue]






% The intensive labor is a central issue in both commercial content moderation [cite] and volunteer content moderation [cite]. 





% Address labor in particular: Besides bringing in algorithm and auto-mod to address harm, the current system can also reduce labor by prevention of harm and reduction of re-offense rate. restorative justice can help with it. (Bring in TJ) It's not only about moderation, it's about culture. The community creates the culture so it has responsibility.



% == design suggestions ==
% bring in elements of restorative justice, instead of restorative justice as a whole, use existing element
% Can offer restorative justice as an alternative

% set separate role of facilitator




% == future work ==
% the types of harm that is suitable for restorative justice
% action research

% \sj{the role platforms must play} look at the paper Shagun sent me

% \ns{commercial content moderation and volunteer moderation --- talk about the two differently. even don't have to give answers, but have to raise the question}
% Platform always hide behind, freedom of speech, etc

% There are problems about format, but change people's notion of justice is the first step

% how do we scale?
% where is the truth finding process?


%\sx{from Richmond: I think maybe one thing to think about framing is did you go in trying to do need-finding for RJ, or did you expect to find RJ already occuring (or both, or neither?)}
% \begin{comment}


% Online platforms generally address those harms through content moderation, where human content moderators, bots and artificial intelligent systems remove offending posts to maintain the health of the content and sometimes ban repeat offenders from the community \cite{lenhart_online_2016}. The current system follows the principles of punitive justice and holds the beliefs that harm is a violation of rules and offenders of harm should suffer in proportion to the offense \cite{garland2012punishment}.
 
% Restorative justice is an alternative approach to address harm. Restorative justice believes that harm is a violation of people and relationships rather than a mere violation of rules \cite{zehr_little_2015}. It puts victims at the center and believes that there is an obligation to repair the harm caused by the wrongful act. There are three major goals of restorative justice: (1) provide support and healing to victims and address their needs in addressing harm, (2) provide offenders a chance to understand how their actions result in harm and take responsibility to repair the harm, and (3) encourage the community to provide support for both victims and offenders, and heal collectively \cite{llewellyn1999restorative}. The primary tool of restorative justice models is communication, often through one-on-one meetings with facilitators and small group conversations that include the person who is harmed and people connected to them as well as the person who caused harm \cite{zehr_little_2015}. During these conversations, participants discuss what harm has happened and how to right the wrong. An agreement is met and signed by all participants.

% In this research, we tries to understand how we can apply restorative justice in online content moderation to address harm. We focused on Overwatch gaming communities and include two places where gamers usually interact: the game Overwatch and social media platform Discord. We interviewed 26 victims of harm, offenders of harm and Discord moderators. There are two goals of our research:
% (1) Understand how different stake holders (victims, offenders and moderators) address harm under the lenses of restorative justice principles.
% (2) Understand people's perspectives on a restorative justice process.

% [add findings and discussion]

% \end{comment}
